The Physics of Mergers: Theoretical and Statistical Techniques Applied to Stellar Mergers in Dense Star Clusters

(abridged) This thesis presents theoretical and statistical techniques broadly related to systems of dynamically-interacting particles composed of several different types of populations. They are applied to observations of dense star clusters (SCs) in order to study gravitational interactions between stars. We present a new analytic method of quantifying the frequency of encounters involving single, binary and triple stars. With this technique, we have shown that dynamical encounters involving triple stars occur commonly in at least some SCs, and that they are likely to be an important dynamical channel for stellar mergers to occur. We have also used our techniques to analyze observational data for a large sample of SCs taken from the ACS Survey for Globular Clusters. The results of this analysis are as follows: (1) We have compiled a homogeneous catalogue of stellar populations for every cluster in our sample, including main-sequence (MS), red giant branch, horizontal branch and blue straggler (BS) stars. (2) With this catalogue, we have quantified the effects of the cluster dynamics in determining the relative sizes and spatial distributions of these stellar populations. (3) These results are particularly interesting for BSs since they provide compelling evidence that they are descended from binary stars. (4) Our analysis of the MS populations is consistent with a remarkably universal initial stellar mass function in old massive SCs in the Milky Way. This is a new result with important implications for our understanding of star formation in the early Universe and, more generally, the history of our Galaxy. Finally, we describe how our techniques are ideally suited for application to a number of other outstanding puzzles of modern astrophysics, including chemical reactions in the interstellar medium and mergers between galaxies in galaxy clusters.

==> SupplementaryMaterial/Dedication.tex <==
\thispagestyle{empty}



%\begin{center}
%\vspace*{1.25in}



%{\it \LARGE\textsf{\`A ma m\`ere Carmelle et mon p\`ere Pierre, que nous
%n'oublirons jamais}}

%\hspace{1.85in}{\it \LARGE\textsf{\`A la m\'emoire de mon p\`ere, Pierre}\\}

\hspace{1.85in}{\it \LARGE\textsf{To my parents}\\}

%\vspace{0.25in}
%{\it \`A ma ch\`ere m\`ere, Carmelle}



%\end{center}
